Revolutionizing Database Q&A with Large Language Models: Comprehensive Benchmark and Evaluation

The development of Large Language Models (LLMs) has revolutionized QA across various industries, including the database domain. However, there is still a lack of a comprehensive benchmark to evaluate the capabilities of different LLMs and their modular components in database QA. To this end, we introduce DQABench, the first comprehensive database QA benchmark for LLMs. DQABench features an innovative LLM-based method to automate the generation, cleaning, and rewriting of evaluation dataset, resulting in over 200,000 QA pairs in English and Chinese, separately. These QA pairs cover a wide range of database-related knowledge extracted from manuals, online communities, and database instances. This inclusion allows for an additional assessment of LLMs' Retrieval-Augmented Generation (RAG) and Tool Invocation Generation (TIG) capabilities in the database QA task. Furthermore, we propose a comprehensive LLM-based database QA testbed DQATestbed. This testbed is highly modular and scalable, with basic and advanced components such as Question Classification Routing (QCR), RAG, TIG, and Prompt Template Engineering (PTE). Moreover, DQABench provides a comprehensive evaluation pipeline that computes various metrics throughout a standardized evaluation process to ensure the accuracy and fairness of the evaluation. We use DQABench to evaluate the database QA capabilities under the proposed testbed comprehensively. The evaluation reveals findings like (i) the strengths and limitations of nine LLM-based QA bots and (ii) the performance impact and potential improvements of various service components (e.g., QCR, RAG, TIG). Our benchmark and findings will guide the future development of LLM-based database QA research.

==> ole_version/5_Evaluation.tex <==
\section{\bench Evaluation Pipeline}\label{sec:pipeline}
We make two lines of effort toward building a thorough, precise and impartial evaluation of question-answering databases (DBs). (1) modularized evaluation protocols and metrics, which rigorously assess intermediate stages such as DB document retrieval, tool selection and tool utilization; and (2) a standardized end-to-end evaluation that ensures stability and control.

\subsection{Modularized Evaluation}

\noindent \textbf{QCR Evaluation. }
Accuracy is the most critical metric when evaluating the QCR module. If the questions are not accurately categorized, the LLM can not provide customized responses. Given the ground truth class labels mentioned in Section~\ref{sec:qcr}, the accuracy is defined as $Acc=\sum_{i} m_{i,i}/\sum_{i} \sum_{j} m_{i,j}$, where $m_{i,j}$ is the number of queries that belong to ground truth class $i$ that are classified as class $j$. We will also report the F1 result of each category $i$ in the experiment as $F1(i) = 2(precision(i)\cdot recall(i))/(precision(i)+recall(i))$. where $precision(i) = m_{i,i}/\sum_{j} m_{i,j}$ and $recall(i) = m_{i,i}/\sum_{j} m_{j,i}$.

\noindent \textbf{RAG Evaluation. }
Firstly, the performance of RAG can be measured by how precise the retrieval is, i.e., whether the retrieval text is relevant to the question. Thus, we can use the P@n metric. In particular, given that the relevance of external knowledge is crucial to the answer quality, we consider only the top three retrieval results. The precision of the RAG module is defined as $P@3 = \sum_{i\leq 3} I\{r_{i,j}\}/(3 \sum_j)$, where $r_{i,j}$ is the $i-$th ranked text block in the top-3 retrieval results of query $j$, and $I\{\}$ is an indicator function that returns whether the text block is relevant as labeled in the retrieval annotation in Section~\ref{sec:bench}, $\sum_j$ means the RAG module's performance is averaged over all queries. 

Secondly, the RAG module in the testbed is optional. The LLM can properly function without RAG or with incorrect RAG results. Therefore, we can also evaluate the performance of the RAG module by comparing the end-to-end performance with and without RAG.


\noindent \textbf{TIG Evaluation. }
The TIG module enhances the LLM by calling appropriate database tools and utilizing the interaction results between the tools and database instances. Two core dimensions need to be measured: (1) Can TIG select the correct set and order of tools for the query? (2) Can TIG correctly trigger the tool, i.e., does the tool invocation adhere to the prompt and tool format requirements? Therefore, we propose TSA (Tool Selection Accuracy) and TFA (Tool Format Accuracy) to measure these two dimensions respectively.

\textit{(1) TSA:} This metric measures whether the correct tools are chosen to solve problems. It is important to consider the order of actions to measure the DB-specific planning ability. For example, the input of the succeeding tool is usually based on and formulated from the preceding tool's output. Therefore, if there is an error in the current tool invocation, the subsequent tool invocations will no longer be included in the metric calculation. Specifically, the TSA (Tool Selection Accuracy) is defined as:
% \begin{equation}
%     TSA = \frac{\sum_{i\geq 1,j}^{i\leq \min{k_j, I\{t_{k_j,j}\}=0}} I\{t_{i,j}\}}{\sum_j k_j},
% \end{equation}
\begin{equation}
    TSA = \sum_{i\geq 1,j}^{i\leq \min{k_j, I\{t_{k_j,j}\}=0}} I\{t_{i,j}\}\big{/}\sum_j k_j,
\end{equation}
where $t_{i,j}$ is $i-$th tool in COT for the query $j$, $I\{\}$ is an indicator function that returns whether the tool (the name after ``Action") is labeled in the tool annotation in Section~\ref{sec:bench}, and $k_j$ means the number of LLM tool invocations. 
% For example. if the first two tools that the LLM uses are ``[correct, incorrect]", then, regardless of whether there is a third tool call in the ground truth, we compute the accuracy as $0.50$. 

\textit{(2) TFA:} This metric measures the accuracy of the tool invocation format. Due to the diversity and subjectivity of tool format requirements, particularly in the generalized tool section \qa, it is very challenging to assess format compliance using predefined rules. Therefore, we employ GPT-4 as an expert adjudicator model to judge whether tool invocations meet the format requirements. Similarly, we consider the order of tools. 
Specifically, the TFA (Tool Format Accuracy) is defined as:
% \begin{equation}
%     TFA = \frac{\sum_{i\geq 1,j}^{i\leq \min{k_j, G\{t_{k_j,j}\}=0}} G\{t_{i,j}\}}{\sum_j k_j},
% \end{equation}
\begin{equation}
    TFA = \sum_{i\geq 1,j}^{i\leq \min{k_j, G\{t_{k_j,j}\}=0}} G\{t_{i,j}\}\big{/}\sum_j k_j,
\end{equation}
where $t_{i,j}$ is the $i-$th tool in COT for the query $j$, $G\{\}$ is the output of GPT-4 that decides whether the tool input (the content after ``Action\_Input") is correct, and $k_j$ means the number of LLM tool invocations. 

\subsection{End-to-End Evaluation}
LLMs are sensitive to prompt engineering. The choice of wording and structure in prompts can influence the quality of LLM's responses. In our practice, the proposed testbed workflow in Section~\ref{sec:framework} can improve the credibility, relevance and fluency of all tested LLMs. Thus, instead of asking a simple query, we use a standard prompt pipeline to obtain the best output of various LLMs.  

\textbf{Standard Evaluation pipeline.} Since there are multiple intermediate steps in the testbed workflow, it is pivotal to fix some of the steps to reduce unexpected output. We use the ground truth labels in the QCR and RAG modules because these modules can be isolated from the LLMs. For example, correctly associating the question ``Why is SQL query execution slow?" with the `instance-specific' label is essential to trigger the DB tools and produce targeted answers. Nonetheless, the QCR accuracy can be boosted by utilizing a more advanced classifier trained explicitly for the QCR task. Thus, the end-to-end evaluation should not be impacted by whether the LLM to be evaluated can classify the question correctly. The retrieval precision can also be upgraded by using a more advanced retriever. On the contrary, the TIG performance is based on the LLM's ability to plan and utilize DB tools. The problem is that the instance's output may deviate from the ground truth, making it difficult to evaluate the personalized answer. Thus, we standardize the LLM end-to-end evaluation process as follows.

\textit{(1) Standard Question Classification}. We use the ground truth question labels to generate the associated prompt template.

\textit{(2) Standard Retrieval Knowledge}. For product-specific queries, we use the ground truth fine-grained retrieval text and append it to the prompt.

\textit{(3) Standard Tool Result}. For instance-specific queries, we formulate the `Thought-Action-Action\_Input-Observation" chain using the Algorithm \ref{alg: evaluation pipeline}. Given the model $M$ to be evaluated, the tool pool $P$, the question $q$, the prompt template $p_0$, and the ground truth answer and tools invoked in the benchmark (line 1), the LLM's answer is initiated as empty (line 2). We first construct the valid tool set \{\{T\}\} in the prompt to include all tools mentioned in the ground truth answer, along with four randomly selected tools from the tool pool $P$ (line 3). For each tool invocation on the ground truth answer (line 4),  a prompt is constructed using the template and the output of the last invoked tool (line 5), and this prompt is used to obtain an answer from the LLM to extract the next action (line 6). If the answer from the evaluated model $M$ uses the same tool as the benchmark (line 7), the `Observation' part of the benchmark answer is appended to the answer from model $M$ (line 8). If a wrong tool is used, it outputs “Tool Invocation Failure” (line 11), and the process is terminated (line 12).

\begin{algorithm}
\caption{Answer Generation in Instance \qa}\label{alg: evaluation pipeline}
\textbf{Input: }evaluated model $M$; tools\_pool $P$; prompt template $p_0$; question $q$; answer ground truth $\hat{a}$; tool set ground truth $\{t\}$; 

$a_0 \leftarrow \emptyset$;

$T$ = \{$t$\} $\cup$ Random\_Select($P$, 4);

\For{i in range(count(“Action” in $\hat{a}$))}{
$p_i$ = $p_0$($T$,$q$,$a_{i-1}$);

$a_i$["Action"]  = $M$($p_i$).extract();

\If{$a_i$["Action"] == $\hat{a}$[i]["Action"]}{
$a_i$.append($\hat{a}$[i]["Observation"]);

\textbf{Continue};
}
$a_i$.append("Tool Invocation Failure.");

\textbf{Break};
}

\textbf{Return $a_i$}
\end{algorithm}

\noindent \textbf{Metrics.} To ensure a comprehensive end-to-end evaluation, we adopt two metrics, namely WinRate and MCA (Multiple Choice Accuracy), to measure the quality of end-to-end generation. 

\textit{(1) MCA (Multiple-Choice Accuracy):} This metric measures the accuracy of all multiple-choice questions following $MCA =\sum_{i} m_{i,i}/\sum_{i}$ $ \sum_{j} m_{i,j}),$ where $m_{i,j}$ is the number of answers that the ground truth choice is $i$ and the LLM's output is $j$, $i,j \in \{A, B, C, D, others\}$. For MCA, we strictly require the model's output to be one letter by prompt, any deviation is classified as $`others'$ and considered a categorization error.

\textit{(2) WinRate:} This metric compares the quality of two different LLMs, i.e., one is the LLM to be evaluated, and the other is a competitor, using a powerful adjudicator model (such as GPT-4)~\footnote{Detailed prompts for WinRate, can be found at \href{https://github.com/XMUDM/DQABench}{[link]}.}. In this study, we use the most common LLM, GPT-3.5, as the competitor for comparison. We calculate WinRate as follows:
\begin{equation}
WinRate = \frac{N_{r=1}}{N_{r=1} + N_{r=-1}}, \quad \text{where} \left\{
\begin{array}{ll}
r = 1 & \text{if } M \text{ wins}, \\
r = 0 & \text{if } M \text{ ties}, \\
r = -1 & \text{if } M \text{ loses},
\end{array}
\right. 
\end{equation} where $N_r$ represents the number of comparisons where the judge GPT-4 considers case $r$, and $M$ is the model to be evaluated. We meticulously designed the judge's prompt so that it uses the answer provided by \bench as the ground truth and deems any response that contradicts the facts as a loser.



==> ole_version/6_Experiment.tex <==
\section{Experiment}\label{sec:exp}

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2pt}
\caption{WinRate of different LLMs versus the competitor}
\label{tab:main_WinRate_Result}
\vspace{-1em}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{lrr|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{$|\boldsymbol{\theta}|$} & \multirow{2}{*}{\textbf{Deployment}} & \multicolumn{2}{c|}{\textbf{DB General}} & \multicolumn{2}{c|}{\textbf{Product-specific}} & \multicolumn{2}{c|}{\textbf{Instance-specific}} & \multicolumn{2}{c}{\textbf{Average}}\\
\cmidrule{4-11}
& & & ZH & EN & ZH & EN & ZH & EN & ZH & EN \\
\midrule
\multicolumn{10}{c}{\texttt{WinRate v.s. Vanilla GPT-3.5-Turbo}} \\
\midrule
\href{https://platform.openai.com/docs/models/gpt-4-turbo-and-gpt-4}{GPT-4} &  & Centralized & \hl{0.85} & \hl{0.95} & 0.86 & \hl{0.86} & 0.69 & 0.53 & \hl{\textbf{0.80}} & \hl{\textbf{0.78}}\\
\href{https://platform.openai.com/docs/models/gpt-3-5-turbo}{GPT-3.5-Turbo} & & Centralized & 0.53 & 0.56 & 0.60 & 0.60 & 0.58 & 0.57 & \textbf{0.57} & \textbf{0.58}\\
\href{https://chatglm.cn/main/detail}{GLM-3-Turbo} & & Centralized & 0.63 & 0.62 & 0.81 & 0.58 & 0.44 & 0.44 & \textbf{0.63} & \textbf{0.55}\\
\href{https://huggingface.co/meta-llama/Meta-Llama-3-8B-Instruct}{Llama3} & 8B & $\geq$RTX 3090 & 0.60 & 0.67 & 0.79 & 0.75 & 0.37 & 0.40 & \textbf{0.59} & \textbf{0.61}\\
\href{https://huggingface.co/meta-llama/Llama-2-13b-chat-hf}{Llama2} & 13B & $\geq$RTX 4090 & 0.12 & 0.09 & 0.35 & 0.41 & 0 & 0 & \textbf{0.16} & \textbf{0.17}\\
\href{https://huggingface.co/IEITYuan/Yuan2-2B-Februa-hf}{Yuan2} & 2B & $\geq$RTX 3060 & 0.03 & 0.02 & 0.22 & 0.18 & 0 & 0 & \textbf{0.08} & \textbf{0.07}\\
\href{https://huggingface.co/baichuan-inc/Baichuan2-13B-Chat}{Baichuan2}(vanilla) & 13B & $\geq$RTX 4090 & 0.27 & 0.29 & 0.56 & 0.60 & 0.23 & 0.15 & \textbf{0.35} & \textbf{0.35}\\
Baichuan2-sft & 13B & $\geq$RTX 4090 & 0.44 & 0.31 & 0.88 & 0.76 & 0.90 & 0.82 & \textbf{0.74} & \textbf{0.63} \\
Imp. w.r.t. vanilla & & & \grey{+0.17} & \grey{+0.02} & \grey{+0.32} & \grey{+0.16} & \grey{+0.67} & \grey{+0.67}& \grey{+0.39} & \grey{+0.28}\\
Baichuan2-cpt-sft & 13B & $\geq$RTX 4090 & 0.57 & 0.48 & \hl{0.88} & 0.74 & \hl{0.91} & \hl{0.87} & \textbf{0.79} & \textbf{0.70}\\
Imp. w.r.t. vanilla & & & \grey{+0.30} & \grey{+0.19} & \grey{+0.32} & \grey{+0.14}  & \grey{+0.68} & \grey{+0.72}& \grey{+0.44} & \grey{+0.35}\\
\midrule
\multicolumn{10}{c}{\texttt{WinRate v.s. GPT-3.5-Turbo (Testbed)}} \\
\midrule
\href{https://platform.openai.com/docs/models/gpt-4-turbo-and-gpt-4}{GPT-4} & & Centralized  & \hl{0.83} & \hl{0.95} & 0.64 & 0.68 & 0.90 & 0.64 & \hl{\textbf{0.79}} & \hl{\textbf{0.76}}\\
\href{https://platform.openai.com/docs/models/gpt-3-5-turbo}{GPT-3.5-Turbo} & &Centralized &- & - & - & - & - & - & - & -\\
\href{https://chatglm.cn/main/detail}{GLM-3-Turbo} & &Centralized & 0.62 & 0.65 & 0.66 & 0.57 & 0.55 & 0.49 &\textbf{0.61} & \textbf{0.57}\\
\href{https://huggingface.co/meta-llama/Meta-Llama-3-8B-Instruct}{Llama3} & 8B & $\geq$RTX 3090 & 0.60 & 0.65 & 0.62  & 0.51 & 0.49 & 0.52 & \textbf{0.57} & \textbf{0.56}\\ 
\href{https://huggingface.co/meta-llama/Llama-2-13b-chat-hf}{Llama2} & 13B & $\geq$RTX 4090 & 0.12 & 0.06 & 0.36 & 0.16 & 0 & 0 & \textbf{0.16} & \textbf{0.07}\\
\href{https://huggingface.co/IEITYuan/Yuan2-2B-Februa-hf}{Yuan2} & 2B & $\geq$RTX 3060 & 0.03 & 0.02 & 0.13 & 0.07 & 0 & 0 & \textbf{0.05} & \textbf{0.03}\\
\href{https://huggingface.co/baichuan-inc/Baichuan2-13B-Chat}{Baichuan2(vanilla)} & 13B & $\geq$RTX 4090 & 0.26 & 0.30 & 0.42 & 0.40 & 0.16 & 0.11 & \textbf{0.28} & \textbf{0.27}\\
Baichuan2-sft & 13B & $\geq$RTX 4090  & 0.44 & 0.30 & \hl{0.68} & 0.66 & 0.85 & 0.87 & \textbf{0.66} & \textbf{0.61} \\
Imp. w.r.t. vanilla & & & \grey{+0.18} & \grey{0} & \grey{+0.26} & \grey{+0.26} & \grey{+0.69} & \grey{+0.76} & \grey{+0.38} & \grey{+0.34} \\
Baichuan2-cpt-sft & 13B & $\geq$RTX 4090 & 0.55 & 0.42 & 0.65 & \hl{0.73} & \hl{0.95} & \hl{0.90} & \textbf{0.72} & \textbf{0.68} \\
Imp. w.r.t. vanilla & & & \grey{+0.29} & \grey{+0.12} &\grey{+0.23} & \grey{+0.33} & \grey{+0.79} & \grey{+0.79}& \grey{+0.44} & \grey{+0.41}\\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table*}


In this section, we focus on the following research questions: 

\noindent \textbf{RQ1:} How do popular general-purpose LLMs perform on \bench? 

\noindent \textbf{RQ2:} How do auxiliary modules on the testbed perform? 

To answer RQ1, we comprehensively evaluate seven popular LLMs by \bench in Section \ref{sec:exp_main} and construct fine-grained analysis in Section \ref{sec:exp_general}. To answer RQ2, we validate pre-training and fine-tuning in Section \ref{sec:exp_main}, QCR evaluation in Section \ref{sec:exp_qcr}, RAG ablation in Section \ref{sec:exp_rag} and TIG evaluation in Section \ref{sec:exp_tig}.

\subsection{Experimental Setup}\label{sec:exp_setup}

\noindent \textbf{\bench details}. \textit{(1) In product-specific subset}, we choose the database product `openGauss' and its latest documentation as of April 2024. The advantage of 'openGauss' is that our evaluated LLMs have not shown any signs of being specifically trained on the latest detailed documentation of this product, effectively avoiding unfair evaluation due to potential data leakage. \textit{(2) In instance-specific subset}, we created \qa pairs under widely recognized database benchmarks TPC-H, TPC-C and TPC-DS as examples.

\noindent \textbf{Testbed implementation}. \textit{(1) QCR:} For all Chinese classifiers, pretrain model: chinese-xlnet-base, we set the batchsize as 512 and learning rate as 5e-4; for all English classifiers, pretrain model: xlnet-base-cased, we set the batchsize as 256 and learning rate as 5e-5. Each classifier trained for 30 epochs and saved the checkpoint performed best on validation sets. \textit{(2) RAG:} We set the text length to 250 characters per segment and the overlap length to 50 characters between adjacent texts in the knowledge base. For each query, up to 3 vectors from the knowledge base are matched with a similarity threshold 0.5. We use L2 distance for similarity search and the default Flat index. \textit{(3) TIG:} We set the number of random tools in the tool pool (\texttt{\{\{T\}\}} in prompt) to 4. 

\noindent \textbf{LLM training}. The LLM training server is a workstation equipped with eight A100 GPU cards. The pre-training phase comprises two epochs using the collected database-related data. The learning rate is 5e-5 and the batch size is 128. In the fine-tuning phase, General DB Q\&A, Product-specific Q\&A, Instance-specific Q\&A and DB-irrelevant Q\&A is assigned with weights 1:1.5:3:0.5, to account for their importance, data volume and training difficulty. The learning rate is 2e-5 and the batch size is 64.

\subsection{LLMs Evaluation by \bench}\label{sec:exp_main}

We implement and evaluate seven LLMs \textbf{(1) GPT-4~\cite{gpt4}}, the most powerful large-scale LLM currently released by OpenAI, using the GPT-4-0125-preview version. \textbf{(2) GPT-3.5~\cite{chatgpt}}, the most popular large-scale LLM currently released by OpenAI, using the GPT-3.5-turbo-0125 version. \textbf{(3) GLM-3~\cite{glm}}, a popular large-scale LLM for both Chinese and English, released by Zhipu AI. \textbf{(4) Llama3-8B~\cite{llama}}, the latest mid-sized open-source LLM released by Meta AI, claimed to achieve state-of-the-art (SOTA) performance among mid-sized models, using the Llama3-8B-Instruct version. \textbf{(5) Llama2-13B~\cite{llama2}}, the most popular mid-sized open-source LLM released by Meta AI, using the Llama1-13B-Chat version. \textbf{(6) Yuan2-2B~\cite{yuan}}, a popular small-sized open-source model for both Chinese and English, released by IEIT Systems, using the Yuan2-2B-Februa version. \textbf{(7) Baichuan2-13B~\cite{baichuan}}, a popular mid-sized open-source model for both Chinese and English, released by Baichuan Intelligence, using the Baichuan2-13B-Chat version. 

The above LLMs are implemented on the proposed testbed with QCR, RAG and TIG. Limited by training time and cost, we only implement Baichuan2-13B with pre-training and fine-tuning on the testbed, leading to two additional LLM variants. \textbf{(8) Baichuan2-13B-sft}, which is a Baichuan2-13B variant fine-tuned as shown in Section \ref{sec:pretrain}. \textbf{(9) Baichuan2-13B-cpt-sft}, which is a Baichuan2-13B variant pre-trained and fine-tuned as shown in Section \ref{sec:pretrain}. 

We compute the WinRate as described in Section \ref{sec:pipeline} of each LLM versus two competitors. \textit{(1) GPT-3.5-Turbo (Vanilla)}: we input the user's question to GPT-3.5-Turbo without employing any prompts strategy. This result focuses on demonstrating the difference between a dedicated database \qa system (the testbed) and typical LLM applications. \textit{(2) GPT-3.5-Turbo (Testbed)}: we also equip GPT-3.5-Turbo on the testbed. This result emphasizes the inherent capability difference of each LLM. We have the following insights from Table~\ref{tab:main_WinRate_Result}.

\noindent \textbf{I1: Larger model sizes and richer pre-training data contribute to powerful DB general \qa. } GPT-4 has achieved SOTA performance on DB general questions. Generally, among LLMs proposed in the same period, larger model sizes tend to perform better. However, Llama3-8B challenges this trend. As stated in its technical report, Llama3-8B introduced an extensive amount of training data (15 trillion tokens) during pre-training, resulting in logarithmic-scale performance improvements. This enhancement is also evident on the \bench dataset.

%\noindent \textbf{I1: Overall, for general-purpose LLMs, GPT-4 is the most advanced model in database \qa, while Llama3-8B is the most advanced model for edge deployment.} The result shows GPT-4 has achieved SOTA performance on three sub-datasets and in two languages for database \qa. It outperforms the second-best model by a significant margin of 0.18-0.23 (approximately 27\%-33\%). When considering only small-size models, the latest Llama-3, with its extensive pre-training and more efficient architecture, surpasses other LLMs. It outperforms the second-best model by 0.24-0.29 (approximately 68\%-107\%), significantly exceeding the overall performance of the most popular LLM GPT-3.5-turbo.

\noindent \textbf{I2: Domain-specific pre-training and fine-tuning can significantly improve model performance. } The testbed's pre-training and fine-tuning have increased the performance of Baichuan2-13B on all question types. Specifically, the pretraining has increased the average performance by 0.28 to 0.39 (approximately 80\% to 111\%). The fine-tuning has brought significant improvements in answering all questions, with an average overall increase of 0.28 to 0.38 (approximately 80\% to 136\%). Notably, the fine-tuning stage targets to reinforce instruction adherence to specific prompt templates and gives the LLM a strong ability to follow specific instructions, outperforming GPT-4 on the instance-specific subset.

\noindent \textbf{I3: RAG and TIG on the testbed can enhance LLM performance in DB \qa.} Comparing the upper half with the bottom half of Table~\ref{tab:main_WinRate_Result}, we observe that the WinRate has generally decreased because GPT-3.5-Turbo is more competitive after being equipped with the testbed. It shows that, even for a sophisticated large-scale LLM, the RAG and TIG on the testbed can be beneficial. We will discuss the impact of the RAG and TIG modules in more detail in Section \ref{sec:exp_rag} and \ref{sec:exp_tig}.

% \noindent \textbf{I4: Retrieval Augment Generation significantly enhances the ability to \qa depend on domain-specific documents.} The table shows that when the model receives external knowledge provided by RAG, its performance on the "product-specific" subset significantly improves compared to its performance on the "general DB" subset without external knowledge. This is particularly notable for small to medium-sized edge-deployed models, which improve performance by 2x to 9x. We will further discuss the influence of the RAG module by ablation study in Section \ref{sec:exp_rag}.

\noindent \textbf{I4: Small-size general LLM can hardly invoke DB tools}. Among all tested models, Llama2 and Yuan2 lack pre-aligned instruction following, resulting in no tool usage capabilities. Although models like Baichuan2-13B claim to have instruction-following alignment, experimental results show that their model size still significantly limits their tool usage capabilities. This indicates that instruction enhancement for specific tool usage is necessary when deploying small to mid sized models. We will further discuss the accuracy of the TIG module in Section \ref{sec:exp_tig}.


\subsection{In-depth Analysis of Database General \qa}\label{sec:exp_general}
In this section, we analyze the ``DB general`` subset in \bench from two perspectives. There are two types of questions in the subset, namely the subjective questions and the objective questions with multiple choices. 

First, we report the WinRate of various LLMs in answering subjective questions. Specifically, we utilize GPT-4 to assign detailed labels to each question in the ``DB general'' subset, incorporating predefined few-shot labels from the prompt and allowing GPT-4 to generate new labels autonomously~\footnote{The details of the classification prompt can be found at \href{https://github.com/XMUDM/DQABench}{[link]}}. We identify eight most common labels: ``Performance Monitoring and Tuning'', ``Backup and Recovery'', ``Query Optimization'', ``Data Migration'', ``Data Security'', ``Database Design and Deployment'', ``Data Analysis'' and ``SQL Programming''. These labels cover 93.79\% of the questions in the ``DB general'' subset.


\begin{figure}[!t]
  \centering
\includegraphics[width=\linewidth]{figures/exp_general_v2.pdf}
  \vspace{-1em}
  \caption{(a) WinRate and (b) Multi-Choice Accuracy on ``DB General" questions}
  \label{fig:exp_general}
  \vspace{-1em}
\end{figure}

The experimental results, illustrated in Figure~\ref{fig:exp_general} (a)'s radar chart, lead to the following conclusions: (1) Numerically, the response capabilities of different models in each sub-field correlate positively with their model size and overall ability, with no model being highly specialized in any particular field. (2) In terms of shape proportion, the radar charts of GPT-3.5 and GPT-4 are similar, showing balanced capabilities across the eight aspects. In contrast, Llama2, Llama3, Baichuan2 and other models based on the llama architecture display a similar pattern, excelling in Performance Monitoring and Tuning but weaker in SQL Programming. This indicates that GPT series models are better at generating accurate SQL Programming instructions, while llama-based models excel in comprehensive subjective analysis. 

Next, we report the Multiple-Choice Accuracy, which is measured on the objective questions. As shown in Figure~\ref{fig:exp_general} (b), MCA aligns closely with the WinRate on subjective questions. This validates that questions in \bench are set with an appropriate difficulty level and require a good understanding of DB knowledge to answer.

\subsection{Question Classification Models Comparison}\label{sec:exp_qcr}
We use the testing data include DB-related questions from \bench, safe but DB-irrelevant questions from Alpaca~\cite{alpaca} and Longbench~\cite{longbench} and unsafe labeled questions from Safety-Prompts~\cite{safety} and BeaverTails Evaluation~\cite{beavertails}~\footnote{The sources and statistics of the dataset are detailed in \href{https://github.com/XMUDM/DQABench}{[link]}.}. The F1 score for each category, average accuracy and response latency deployed on a workstation with a RTX-3090 GPU card are shown in Table~\ref{exp_qcr}.

\setlength{\tabcolsep}{0.9pt}
\begin{table}[t!]
\centering
\caption{Classification Result by Different Methods}
\label{exp_qcr}
\vspace{-1em}
\begin{tabular}{l|ccccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \ & & \textbf{F1-score} & &  & \multirow{2}{*}{\textbf{ACC}} & \multirow{2}{*}{\textbf{Latency}} \\
& \textbf{Unsafe} & \textbf{General} & \textbf{Gauss} & \textbf{Tool} & \textbf{No-DB} & &  \\
\midrule
 \multicolumn{8}{c}{\textbf{ZH}} \\
\midrule
GPT-4  & 0.77 & 0.48 & 0.47 & 0.25 & 0.59 & \textbf{0.55} &  \textbf{2.64s} \\
Classifier  & 0.95 & 0.89 & 0.92 & 0.91 & 0.79 & \textbf{0.90} & \hl{\textbf{0.39s}} \\
Hierarchical  & 0.95 & 0.91 & 0.98 & 0.99 & 0.87 & \hl{\textbf{0.94}} & \textbf{0.68s} \\
\midrule
 \multicolumn{8}{c}{\textbf{EN}} \\
\midrule
GPT-4 & 0.80 & 0.57 & 0.37 & 0.49 & 0.69  & \textbf{0.63} & \textbf{2.61s} \\
Classifier  & 0.91 & 0.92 & 0.81 & 0.90 & 0.79 & \textbf{0.87} & \hl{\textbf{0.37s}} \\
Hierarchical & 0.92 & 0.97 & 0.88 & 0.93 & 0.91 & \hl{\textbf{0.92}}  & \textbf{0.67s} \\
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

From the experimental results, we have the following conclusions: (1) Training a dedicated model for safety filtering and classification is essential. Even with the most advanced LLM, GPT-4, the accuracy and latency in classification are inferior to those of a well-trained small model. (2) There is a trade-off between latency and performance across different small models. As shown in Table~\ref{exp_qcr}, the hierarchical classifier can achieve approximately a 0.05 performance improvement at the cost of 300ms. 



\subsection{Retrieval Augment Generation Ablation}\label{sec:exp_rag}
To further investigate the impact of the RAG module on DB \qa, we conduct an ablation study on the RAG module. Specifically, based on the experiments described in Section \ref{sec:exp_main}, we conduct experiments for the ``product-specific" sub-dataset without the external knowledge provided by the RAG module. The WinRate results are shown in Figure \ref{fig:exp_rag}. 

\begin{figure}[!t]
  \centering
\includegraphics[width=0.97\linewidth]{figures/exp-RAG.pdf}
  \vspace{-2em}
  \caption{WinRate v.s. GPT-3.5 (Vanilla) with and without RAG}
  \label{fig:exp_rag}
  \vspace{-.5em}
\end{figure}

From the experimental results, we can observe the following: (1) The RAG module significantly enhances the performance of general-purpose LLMs of any model size, consistent with the analysis in Section \ref{sec:exp_main}. (2) The RAG module can boost the performance of small-sized models several times (e.g., 2.4x for Llama2), demonstrating its substantial value for edge deployment models. (3) The RAG module offers smaller performance improvements for models like Baichuan2-sft fine-tuned with domain knowledge in databases. This indicates a high degree of overlap between the improvements from model fine-tuning and those from the RAG module, suggesting that deploying either one is sufficient within a limited budget.


\subsection{Tool Invocation Analysis}\label{sec:exp_tig}
In the experimental setup described in Section \ref{sec:exp_main}, we further evaluated LLMs on the ``instance-specific" sub-dataset for Tool Selection Accuracy (TSA) and Tool Format Accuracy (TFA). The experimental results are shown in Figure \ref{fig:tool}. From the experimental results, we can observe the following: (1) For general-purpose LLMs, the ability to select and correctly format tools is strongly correlated with their overall capabilities. (2) Specific instruction-following fine-tuning is crucial. Llama-2 and Yuan-2, which have not undergone any instruction-following fine-tuning, lack any tool-invocation abilities. In contrast, the Baichuan2-sft model, fine-tuned with specific tool instruction following, achieves excellent performance. (3) The tool accuracy of Baichuan-2-sft even surpasses that of GPT-4. This suggests that in scenarios with limited tools (strong generalization in tool invocation is not required), specific tool instruction-following fine-tuning can significantly adapt LLMs to the task. (4) Further analysis reveals that in WinRate metrics, the expert evaluator GPT-4 consistently favored responses with successful tool calls as winners. This indicates a strong preference for customized answers utilizing tools, not only among humans but also in LLMs.



\begin{figure}[!t]
  \centering
\includegraphics[width=0.95\linewidth]{figures/tool.pdf}
  \vspace{-1em}
  \caption{Performance of TIG by different LLMs}
  \label{fig:tool}
  \vspace{-1em}
\end{figure}










==> ole_version/intro_sigmod.tex <==
\section{Introduction}


\begin{figure*}[!t]
  \centering
 \includegraphics[width=\linewidth]{figures/intro_v9.pdf}
  \caption{Database \qa Classification and Solutions. (a) Percentage of different \qa types in online DB communities. (b-d)  answers given for typical questions by (b) experts, (c) DB bot (vision), (d) general-purpose LLM (GPT-4). }
  \label{fig:intro}
  \vspace{-1em}
\end{figure*}

Databases play a critical role in enterprises. According to Worldmetrics~\cite{worldmetrics}, over 68\% of organizations worldwide utilize multiple DBMS to meet diverse needs. In industries such as finance, biotechnology, and healthcare, more than 10\% of IT budgets are used on the deployment, use, and maintenance of databases. However, deploying, configuring, tuning, and optimizing databases is a tedious process, making it challenging for DBAs to respond swiftly to arising issues. Therefore, there is a need to design an intelligent database \qa bot as a copilot of DBAs. As illustrated in Figure~\ref{fig:intro} (a)\footnote{The distribution is calculated based on $68,801$ questions collected from StackExchange.}, database Q\&As can be generally categorized into (1) \textit{General DB queries}, which involve fundamental concepts in the database domain, e.g., SQL grammar, the definition of the E-R data model. (2) \textit{Product-specific queries}, which relate to the use of particular database products, e.g., set up a local PostgreSQL database, operational instruction for Snowflake. (3) \textit{Instance-specific queries}, which are centered on a particular database instance, e.g., fault diagnosis and data analysis for a bank's database running on Postgres v16 with Intel i7 CPU. 

Traditionally, seeking solutions to these questions is challenging, often requiring users to consult a vast array of textbooks, product documents and search engines. Users also need to repeat manual operations to obtain contextual information and engage in multi-round dialogues. For example, as shown in Figure~\ref{fig:intro} (b), users have great trouble getting the final answer by repeatedly $(i)$ searching diagnosis knowledge and then $(ii)$ verifying in their database environment (e.g., examine error messages or resource usage).

The emergence of Large Language Models (LLMs)~\cite{chatgpt} has revolutionized \qa in various domains, such as medicine~\cite{medicine1,medicine2}, finance~\cite{finance}, earth science~\cite{earth}, law~\cite{law}, etc. 
Our vision for the LLM-based DB \qa bot is that, as shown in Figure~\ref{fig:intro} (c)\footnote{Showcases are abbreviated from answers generated by Baichuan2-cpt-sft 13B, which is Baichuan2 continued-pre-trained, fine-tuned, and enhanced by various modules in our proposed testbed.}, the user only needs to input a query, and the bot will autonomously utilize various external sources such as DBMS manual documents and database instance information to provide a customized and accurate answer.

However, whether the current LLMs can fully realize our vision is unclear. For example, as shown in Figure~\ref{fig:intro} (d)\footnote{Showcases are abbreviated from answers generated by GPT-4.}, even the most popular and powerful LLM (GPT-4) cannot always give correct and targeted answers. There \textit{lacks a comprehensive evaluation of LLMs on DB-specific \qa tasks} that can enable us to understand the challenges and opportunities of database \qa in the era of LLMs. Although numerous research efforts have evaluated LLMs from different aspects, they have not been dedicated to database \qa tasks, and face the following challenges.

\textbf{C1: Database \qa Dataset}. To increase the scalability of manually designed datasets, current evaluations of LLMs are mostly based on data collected from the Internet~\cite{SQuAD,wiki,amazon,reddit}, which has the following issues in the DB domain. (1) \textit{Low Question Quality}.  Online questions are too brief and lack essential contextual information. For example, a question on slow database performance without hardware (CPU, IO) or query information is impossible to diagnose. (2) \textit{Low Answer Quality}. Many online answers are factually incorrect, overly concise, or too subjective. (3) \textit{Limited Diversity}. Due to factors such as conformity bias, questions in online communities like StackOverflow tend to center on a narrow range of topics and DBMS products, e.g., users are too shy to pose ``silly'' questions, or most questions concern popular DBMS products.

\textbf{C2: Database \qa bot testbed}. Previous evaluations of LLM~\cite{datasetSurvey} primarily focus on a standalone LLM. Unfortunately, regardless of the LLM backbone architectures, a series of components are indispensable in a well-designed DB \qa bot system to answer a wide range of DB questions. These components include: \textit{pre-training} to equip the LLM with domain knowledge to answer DB general questions, \textit{fine-tuning} to enhance the LLM to follow DB-specific instructions, \textit{routing} to adopt different reasoning logics for various types of questions, \textit{retrieving} to consult an external product knowledge source to answer product-specific questions, and \textit{tool invocating} to interact with the DB environment to answer instance-specific questions. Thus, a testbed is required to support all LLMs and integrate with these components and fully demonstrate the potential performance of LLMs in the database \qa domain.

\textbf{C3: Database \qa Evaluation.} To comprehensively and accurately assess the capabilities of LLM-based systems in database \qa is no easy task. We need both reasonable and standardized metrics and evaluation processes to measure the end-to-end performance of various popular LLMs, as well as fine-grained evaluation and analysis of each module to highlight the development potential of individual components within LLM systems and reveal the limitations and challenges for existing technical solutions.

To address these challenges, we construct a comprehensive benchmark \bench (Database Question-Answer) and present a thorough evaluation based on \bench.

\textbf{To address C1}, we construct a diverse \qa dataset by enriching queries from online DB resources and enhancing answer quality through cleaning and rewriting. We also apply a few-shot learning and chain-of-thought approach to extract \qa pairs from DBMS documents and instances, increasing dataset diversity. \textbf{To address C2}, we propose a comprehensive testbed that modularizes all components of a complete DB \qa bot, including pre-training, fine-tuning, Question-Category Routing (QCR), Prompt-Template Engineering (PTE), Retriever-Augmented Generation (RAG), and Tool-Invocation Generation (TIG), each optimized to adapt general-purpose LLMs for DB \qa tasks. \textbf{To address C3}, we implement a standardized end-to-end evaluation, which reducing uncertainty in answer comparison for seven popular LLMs and show the impact of pre-training and fine-tuning on LLM capabilities in database \qa. Additionally, we develop a modular evaluation framework to assess both the development potential and current performance of intermediate components such as question classification, document retrieval, and tool usage.

% To address \textbf{C1}, we construct a large \qa dataset with high quality and diversity. We collect a variety of online queries from online DB courses and forums and enrich the queries with contextual details to \textit{enhance question qualities}. We collect, clean and rewrite online answers to \textit{improve answer qualities}. We propose a novel method based on few-shot learning and chain of thought to extract \qa pairs from DBMS documents and instances to \textit{increase \qa diversity} and cover more DBMS products, instances, and tools.

% To address \textbf{C2}, we propose a full-chain testbed that incorporates and modularizes all necessary components of a complete DB \qa bot to handle real-production DB \qa scenarios, including pre-training, fine-tuning, Question-Category Routing (QCR), Prompt-Template Engineering (PTE), Retriever-Augmented Generation (RAG) and Tool-Invocation Generation (TIG). We have improved the implementation of each module to better adapt a general-purpose LLM to the DB \qa task. 

% To address \textbf{C3}, we propose a standardized end-to-end evaluation to reduce uncertainty in comparing unexpected answers with ground truths, revealing the capabilities of different LLMs in the domain of database \qa, as well as the impact of pre-training and fine-tuning techniques. Additionally, we develop a modularized evaluation framework to comprehensively assess both the potential development and the current performance of intermediate steps, including question classification, database document retrieval and tool utilization.

In summary, we make the following contributions. 

(1) We propose the first benchmark dataset \bench in the database \qa domain. To simulate real-world DB scenarios and cover a wide spectrum of questions, including questions regarding DB general knowledge and complex questions that demand assistance from external manuals and DB tools. The dataset is large-scale with 200,000 \qa pairs, larger than existing instruction datasets in the IT domain~\cite{datasetSurvey}. (Section \ref{sec:bench})

(2) We propose a plug-and-play testbed to experiment with different LLM application strategies. The testbed encapsulates all components potentially involved in the database \qa, such as Question-Categorization Routing (QCR), Prompt-Template Engineering (PTE), Retriever-Augmented Generation (RAG) and Tool-Invocation Generation (TIG).  (Section \ref{sec:framework})

(3) We conducted comprehensive evaluations at both the end-to-end level and the modular level using the \bench dataset and our proposed testbed, which includes seven popular LLMs and two trained and fine-tuned variants. Our end-to-end evaluation demonstrated the capabilities of diverse LLMs, while our modular analysis delved into the contributions of individual components. We discovered and quantified several insights, including but not limited to the following five key areas: (Section \ref{sec:end2end} and \ref{sec: modular})

\noindent \textbf{I1: Capabilities of Diverse LLMs. }We find large language models show a wide disparity in their performance on database QA tasks. lower-performing ones are almost entirely incapable of handling advanced tasks such as tool usage and understanding lengthy retrieval documents. Moreover, we found that larger model sizes and richer pre-training datasets consistently lead to better performance, regardless of which sub-field of database QA is being considered.

\noindent \textbf{I2: Pre-training and Fine-tuning. }Pre-training and Fine-Tuning: Pre-training plays a crucial role in developing a broad understanding of database-related knowledge, whereas fine-tuning significantly enhances performance across all tasks, especially those requiring instruction-following abilities, such as tool invocation.

\noindent \textbf{I3: Question Classification Routing. }We verified that the QCR module is crucial for generating custom responses. Moreover, we explored different implementations and concluded that future designs should focus on well-trained small classification models rather than relying on LLMs for direct response generation.

\noindent \textbf{I4: Retrieval Augment Generation. }we validated the potential of RAG module effectively enhances the LLM’s response by leveraging document retrieval. Moreover, we explored different existing solutions and identified that the primary bottleneck lies in improving the recall rate of the retrieval model, rather than optimizing the interaction between the retrieval module and the LLM.

\noindent \textbf{I5: Tool Invocation Generation. }We validated the potential of the TIG module in enhancing LLM responses through tool invocation. Furthermore, we identified that the key bottleneck of TIG performance is improving the accuracy of tool selection and invocation, both of which are highly dependent on the model's instruction-following capabilities.

% (3) We conduct comprehensive end-to-end evaluations using the \bench dataset and the proposed testbed for seven popular LLMs, along with two trained and fine-tuned variants. We discovered and quantified several insights, including but not limited to: (a) Larger model sizes and richer training data generally lead to better performance across the seven LLMs. (b) Pretraining can improve general DB knowledge understanding, while fine-tuning can significantly enhance all aspect of performance, particularly in instruction-following tasks like tool invocation. (c) There is substantial overlap in the performance gains from pretraining, fine-tuning, and the RAG module, etc. (Section \ref{sec:end2end})

% (4) We conducted a detailed modular analysis of components in the proposed testbed. We demonstrated the necessity of the QCR, RAG, and TIG modules for database QA in terms of their potential to improve performance. Additionally, we evaluated the current technologies in each module to identify future directions for improvement, e.g., (a) the QCR module should focus on using lightweight classification models instead of relying on LLM responses, (b) the main bottleneck for the RAG module lies in enhancing the retrieval model's recall rate rather than the interactive technology between the retrieval module and LLM, and (c) the TIG module's performance depends on accurate tool selection and correct invocation, which highlights that effective instruction-following is key to its performance, etc. (Section \ref{sec: modular})



==> tables/classification_result.tex <==
\setlength{\tabcolsep}{0.9pt}
\begin{table}[t!]
\centering
\caption{Classification Result for Different Methods}
\label{exp_qcr}
\vspace{-1em}
\begin{tabular}{l|ccccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \ & & \textbf{F1-score} & &  & \multirow{2}{*}{\textbf{ACC}} & \multirow{2}{*}{\textbf{Latency}} \\
& \textbf{Unsafe} & \textbf{General} & \textbf{Gauss} & \textbf{Tool} & \textbf{No-DB} & &  \\
\midrule
 \multicolumn{8}{c}{\textbf{ZH}} \\
\midrule
llm-based  & 0.77 & 0.48 & 0.47 & 0.25 & 0.59 & \textbf{0.55} &  \textbf{2.64s} \\
multi-step  & 0.95 & 0.91 & 0.98 & 0.99 & 0.87 & \hl{\textbf{0.94}} & \textbf{0.68s} \\
one-step  & 0.95 & 0.89 & 0.92 & 0.91 & 0.79 & \textbf{0.90} & \hl{\textbf{0.39s}} \\
\midrule
 \multicolumn{8}{c}{\textbf{EN}} \\
\midrule
llm-based & 0.80 & 0.57 & 0.37 & 0.49 & 0.69  & \textbf{0.63} & \textbf{2.61s} \\
multi-step & 0.92 & 0.97 & 0.88 & 0.93 & 0.91 & \hl{\textbf{0.92}}  & \textbf{0.67s} \\
one-step  & 0.91 & 0.92 & 0.81 & 0.90 & 0.79 & \textbf{0.87} & \hl{\textbf{0.37s}} \\
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

==> tables/dataset_statistic.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[!t]
  \caption{Dataset in \bench}
  \label{tab:test}
  \vspace{-1em}
\begin{tabular}{llll}
    \toprule
   Dataset Type & Source & Count & Additional Info \\
    \midrule
   General Knowledge & Multiple Choice &  1946 & Result Explanation\\
    & StackOverflow &  15051 & - \\
   & StackExchange& 53751 & -\\
   & MoDB & 5920 & -\\
   Product-specific & openGauss & 21692 & Retrieval Text \\
   & GaussDB & 4953 & Retrieval Text  \\
Instance-specific& Tools-based & 1084 & Instance\&Tool Info \\
   & Scenarios-based & 2714 &  Instance\&Tool Info\\
  \bottomrule  
\end{tabular}
  \vspace{-1em}
\end{table}

==> tables/framework_comparison.tex <==
\begin{table}[!t]
    \centering
    \caption{Comparison of LLM-based Database QA Solutions}
    \label{tab:framework}
    \vspace{-1em}
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
        \thead{\textbf{Solution}} & \thead{\textbf{Pre-} \\ 
        \textbf{training}} & \thead{\textbf{Fine-} \\ \textbf{tuning}} & \thead{\textbf{Question} \\ \textbf{Classification}} & \thead{\textbf{Retrieval} \\ \textbf{Augment}} & \thead{\textbf{Tool/} \\ \textbf{Agent}} \\
        \midrule
        LLM-only & $\checkmark$ & $\checkmark$ & X & X & X \\
        Langchain~\cite{langchain} & X & X & X & $\checkmark$ & O \\
        D-bot~\cite{db-gpt-zhou} & X & X & X & $\checkmark$ & O+ \\
        DB-GPT~\cite{db-gpt-xue} & X & $\checkmark$ & X & $\checkmark$ & O+ \\  
        \textbf{Ours} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
        \bottomrule
    \end{tabular}
    \smallskip
\parbox{0.95\linewidth}{\small \textbf{Note:} $\checkmark$: Fully supports the component; O+: Can implement but lacks comprehensive implementation; O: Can implement but not any implementation on database \qa; X: Lacks functionality completely.}
\vspace{-2em}
\end{table}

==> tables/main_WinRate_result.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2pt}
\caption{
\textbf{Evaluated Model v.s. GPT-3.5-turbo WinRate Result.} \textit{(1) Naive:} We input the user's question to GPT-3.5-Turbo without employing any prompts strategy. This result focuses on demonstrating the difference between a dedicated database \qa system (the testbed) and typical LLM applications. \textit{(2) Equipped:} We also equipped GPT-3.5-Turbo on the testbed for fair comparison. This result emphasizes the inherent capability difference of each LLM.
}
\label{tab:main_WinRate_Result}
\vspace{-1em}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{lrr|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{$|\boldsymbol{\theta}|$} & \multirow{2}{*}{\textbf{Deployment}} & \multicolumn{2}{c|}{\textbf{General Knowledge}} & \multicolumn{2}{c|}{\textbf{Specific Product}} & \multicolumn{2}{c|}{\textbf{Specific Instance}} & \multicolumn{2}{c}{\textbf{AVG}}\\
\cmidrule{4-11}
& & & ZH & EN & ZH & EN & ZH & EN & ZH & EN \\
\midrule
\multicolumn{10}{c}{\texttt{WinRate v.s. Naive GPT-3.5-Turbo}} \\
\midrule
\href{https://platform.openai.com/docs/models/gpt-4-turbo-and-gpt-4}{GPT-4} &  & Centralized & \hl{0.85} & \hl{0.95} & 0.86 & \hl{0.86} & 0.69 & 0.53 & \hl{\textbf{0.80}} & \hl{\textbf{0.78}}\\
\href{https://platform.openai.com/docs/models/gpt-3-5-turbo}{GPT-3.5-Turbo} & & Centralized & 0.53 & 0.56 & 0.60 & 0.60 & 0.58 & 0.57 & \textbf{0.57} & \textbf{0.58}\\
\href{https://chatglm.cn/main/detail}{GLM-3-Turbo} & & Centralized & 0.63 & 0.62 & 0.81 & 0.58 & 0.44 & 0.44 & \textbf{0.63} & \textbf{0.55}\\
\href{https://huggingface.co/meta-llama/Meta-Llama-3-8B-Instruct}{Llama3} & 8B & $\geq$RTX 3090 & 0.60 & 0.67 & 0.79 & 0.75 & 0.37 & 0.40 & \textbf{0.59} & \textbf{0.61}\\
\href{https://huggingface.co/meta-llama/Llama-2-13b-chat-hf}{Llama2} & 13B & $\geq$RTX 4090 & 0.12 & 0.09 & 0.35 & 0.41 & 0 & 0 & \textbf{0.16} & \textbf{0.17}\\
\href{https://huggingface.co/IEITYuan/Yuan2-2B-Februa-hf}{Yuan2} & 2B & $\geq$RTX 3060 & 0.03 & 0.02 & 0.22 & 0.18 & 0 & 0 & \textbf{0.08} & \textbf{0.07}\\
\href{https://huggingface.co/baichuan-inc/Baichuan2-13B-Chat}{Baichuan2} & 13B & $\geq$RTX 4090 & 0.27 & 0.29 & 0.56 & 0.60 & 0.23 & 0.15 & \textbf{0.35} & \textbf{0.35}\\
Baichuan2-sft & 13B & $\geq$RTX 4090 & 0.44 & 0.31 & 0.88 & 0.76 & 0.90 & 0.82 & \textbf{0.74} & \textbf{0.63} \\
$\Delta$ & & & \grey{+0.17} & \grey{+0.02} & \grey{+0.32} & \grey{+0.16} & \grey{+0.67} & \grey{+0.67}& \grey{+0.39} & \grey{+0.28}\\
Baichuan2-cpt-sft & 13B & $\geq$RTX 4090 & 0.57 & 0.48 & \hl{0.88} & 0.74 & \hl{0.91} & \hl{0.87} & \textbf{0.79} & \textbf{0.70}\\
$\Delta$ & & & \grey{+0.30} & \grey{+0.19} & \grey{+0.32} & \grey{+0.14}  & \grey{+0.68} & \grey{+0.72}& \grey{+0.44} & \grey{+0.35}\\
\midrule
\multicolumn{10}{c}{\texttt{WinRate v.s. GPT-3.5-Turbo Equipped on Testbed}} \\
\midrule
\href{https://platform.openai.com/docs/models/gpt-4-turbo-and-gpt-4}{GPT-4} & & Centralized  & \hl{0.83} & \hl{0.95} & 0.64 & 0.68 & 0.90 & 0.64 & \hl{\textbf{0.79}} & \hl{\textbf{0.76}}\\
\href{https://platform.openai.com/docs/models/gpt-3-5-turbo}{GPT-3.5-Turbo} & &Centralized &- & - & - & - & - & - & - & -\\
\href{https://chatglm.cn/main/detail}{GLM-3-Turbo} & &Centralized & 0.62 & 0.65 & 0.66 & 0.57 & 0.55 & 0.49 &\textbf{0.61} & \textbf{0.57}\\
\href{https://huggingface.co/meta-llama/Meta-Llama-3-8B-Instruct}{Llama3} & 8B & $\geq$RTX 3090 & 0.60 & 0.65 & 0.62  & 0.51 & 0.49 & 0.52 & \textbf{0.57} & \textbf{0.56}\\ 
\href{https://huggingface.co/meta-llama/Llama-2-13b-chat-hf}{Llama2} & 13B & $\geq$RTX 4090 & 0.12 & 0.06 & 0.36 & 0.16 & 0 & 0 & \textbf{0.16} & \textbf{0.07}\\
\href{https://huggingface.co/IEITYuan/Yuan2-2B-Februa-hf}{Yuan2} & 2B & $\geq$RTX 3060 & 0.03 & 0.02 & 0.13 & 0.07 & 0 & 0 & \textbf{0.05} & \textbf{0.03}\\
\href{https://huggingface.co/baichuan-inc/Baichuan2-13B-Chat}{Baichuan2} & 13B & $\geq$RTX 4090 & 0.26 & 0.30 & 0.42 & 0.40 & 0.16 & 0.11 & \textbf{0.28} & \textbf{0.27}\\
Baichuan2-sft & 13B & $\geq$RTX 4090  & 0.44 & 0.30 & \hl{0.68} & 0.66 & 0.85 & 0.87 & \textbf{0.66} & \textbf{0.61} \\
$\Delta$ & & & \grey{+0.18} & \grey{0} & \grey{+0.26} & \grey{+0.26} & \grey{+0.69} & \grey{+0.76} & \grey{+0.38} & \grey{+0.34} \\
Baichuan2-cpt-sft & 13B & $\geq$RTX 4090 & 0.55 & 0.42 & 0.65 & \hl{0.73} & \hl{0.95} & \hl{0.90} & \textbf{0.72} & \textbf{0.68} \\
$\Delta$ & & & \grey{+0.29} & \grey{+0.12} &\grey{+0.23} & \grey{+0.33} & \grey{+0.79} & \grey{+0.79}& \grey{+0.44} & \grey{+0.41}\\
\bottomrule
\end{tabular}
}
\end{table*}

% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{2pt}
% \caption{
% \textbf{Evaluated Model v.s. GPT-3.5-turbo WinRate Result.} We experimented with two strategies for comparing against GPT-3.5-Turbo: (1) Naive: We simply input the user's question to GPT-3.5-Turbo without employing any prompts strategy. This benchmark focuses on demonstrating difference for a dedicated database QA system and typical LLM applications. (2) Knowledge: We equipped GPT-3.5-Turbo with the same prompts and module as the evaluated model to enable fair comparison under the Knowledge condition. This benchmark emphasizes the inherent capabilities of each LLM.
% }
% \label{tab:main_WinRate_Result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lrcrr|ccccccccc|c}
% \toprule
% \textbf{Model} & $|\boldsymbol{\theta}|$ & \textbf{Data} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Uniq.\\ Toks$^*$\end{tabular}}}& \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Toks\end{tabular}}} & \textbf{GSM8K} & \textbf{MATH$^\dagger$} & \textbf{SVAMP} & \textbf{ASDiv} & \textbf{MAWPS} & \textbf{TAB}& \textbf{MQA} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MMLU\\ STEM\end{tabular}}} & \textbf{SAT$^\ddagger$} & \textbf{AVG} \\
% \midrule
% \multicolumn{15}{c}{\texttt{1-2B Base Models}} \\
% \midrule
% \href{https://huggingface.co/Tinyllama/Tinyllama-1.1B-intermediate-step-1431k-3T}{Tinyllama}& 1.1B & - & - & - & 2.9 & 3.2 & 11.0 & 18.1 & 20.4 & 12.5 & 14.6 & 16.1 & 21.9 & 13.4 \\
% \href{https://huggingface.co/microsoft/phi-1_5}{Phi-1.5} & 1.3B & - & - & - & 32.4 & 4.2 & 43.4 & 53.1 & 66.2 & 24.4 & 14.3 & 21.8 & 18.8 & 31.0 \\
% \href{https://huggingface.co/Qwen/Qwen1.5-1.8B}{Qwen1.5} & 1.8B & - & - & - & \hlb{36.1} & 6.8 & \hlb{48.5} & \hlb{63.6} & \hlb{79.0} & 29.2 & 25.1 & 31.3 & 40.6 & \hlb{40.0} \\
% \href{https://huggingface.co/google/gemma-2b}{Gemma} & 2.0B & - & - & - & 18.8 & 11.4 & 38.0 & 56.6 & 72.5 & \hlb{36.9} & \hlb{26.8} & \hlb{34.4} & 50.0 & 38.4 \\ 
% % \href{https://huggingface.co/openbmb/MiniCPM-2B-sft-bf16}{MiniCPM} & 2.4B& - & - & - & 52.7 & 16.0 & 67.0 & 73.2 & 90.1 & 37.6 & 40.9 & 43.1 & 46.9 & 51.9 \\
% % \href{https://huggingface.co/microsoft/phi-2}{Phi2} & 2.7B & - & - & - & 55.3 & 11.8 & 65.4 & 75.5 & 84.0 & 43.6 & 38.2 & 47.9 & 40.6 & 51.4 \\
% DeepSeekLLM & 1.3B & OWM & 14B & 150B & 11.5 & 8.9 & - & - & - & -  & - & 29.6 & 31.3 & -\\
% % DeepSeekLLM-1.3B & Proof-Pile-2 & 55B & 150B & 14.3 & 11.2 & - & - & - & - \\
% DeepSeekMath & 1.3B & - & 120B & 150B & 23.8 & \hlb{13.6} & - & - & - & - & - & {33.1} & \hlb{56.3} & - \\
% \midrule
% \multicolumn{15}{c}{\texttt{Continual Pretraining on Tinyllama-1B}}
% \\ \midrule
% % Tinyllama-1B & Proof-Pile-2 & 55B & 100B & 8.9 & 6.0 & 25.6 & 42.1 & 53.6 & 27.2 \\
% Tinyllama-CT & 1.1B & OWM & 14B & 15B & 6.4 & 2.4 & 21.7 & 36.7 & 47.7 & 17.9 & 13.9 & 23.0 & 25.0 & 21.6 \\
% -Math & 1.1B & OWM & 14B & {9B} & 29.8 & 14.0 & 49.2 & 61.4 & 79.8 & 25.8 & 30.4 & \hl{24.7} & 28.1 & 38.1 \\
% $\Delta$  & & & & \grey{-40\%} & \blue{+23.4} & \blue{+11.6} & \blue{+27.5} & \blue{+24.7} & \blue{+32.1} & \blue{+7.9} & \blue{+16.5} & \blue{+1.7} & \blue{+3.1} & \blue{\textbf{+16.5}} \\
% % {-Math t4} & 1.1B & OWM & 14B & {9B} & 30.1 & 12.2 & 45.4 & 60.1 & 77.6 & 22.6 & 27.3 & \hl{24.1} & 24.0 & 35.9\\
% % $\Delta$ T4 & & & & \grey{-6B} & \blue{+23.7} & \blue{+9.8} & \blue{+23.7} & \blue{+23.4} & \blue{+29.9} & \blue{+4.7} & \blue{+13.4} & \blue{+1.1} & \blue{-1.0} & \blue{\textbf{+14.3}}\\  
% \midrule
% -Math & 1.1B & OWM & 14B & {30B} & \hl{36.2} & \hl{15.6} & \hl{52.1} & \hl{67.0} & \hl{83.9} & \hl{29.0} & \hl{32.5} & {23.3} & \hl{28.1} & \hl{40.9} \\
% \midrule
% \multicolumn{15}{c}{\texttt{$\ge$ 7B Base Models}}
% \\ \midrule
% \href{https://huggingface.co/meta-llama/Llama-2-7b-hf}{LLaMA-2} & 7B & & - & - & 14.0 & 3.6 & 39.5 & 51.7 & 63.5 & 30.9 & 12.4 & 32.7 & 34.4 & 31.4 \\
% % \href{https://huggingface.co/codellama/CodeLlama-7b-Python-hf}{CodeLlama} & 7B & & - & - & 12.4 & 7.0 & 44.5 & 49.0 & 64.9 & 25.5 & 17.2 & 24.1 & 34.4 & 31.0 \\ 
% \href{https://huggingface.co/mistralai/Mistral-7B-v0.1}{Mistral} & 7B & & - & - & 41.2 & 11.6 & 64.7 & 68.5 & 87.5 & 52.9 & 33.0 & 49.5 & 59.4 & 52.0 \\
% Minerva & 8B & - & 39B & 164B & 16.2 & 14.1 & -& -& -& -& -& 35.6 & - & - \\
% Minerva & 62B & - & 39B & 109B & 52.4 & 27.6 & -& -& -& -& -& 53.9 & - & - \\
% Minerva & 540B & - & 39B & 26B & 58.8 & {33.6} & -& -& -& -& -& \hlb{63.9} & - & - \\
% \href{https://huggingface.co/EleutherAI/llemma_7b}{LLemma} & 7B & PPile & 55B & 200B & 38.8 & 17.2 & 56.1 & 69.1 & 82.4 & 48.7 & 41.0 & 45.4 & 59.4 & 50.9 \\
% \href{https://huggingface.co/EleutherAI/llemma_34b}{LLemma} & 34B & PPile & 55B & 50B & 54.2 & 23.0 & 67.9 & {75.7} & 90.1 & 57.0 & 49.8 & 54.7 & 68.8 & 60.1 \\
% \href{https://huggingface.co/internlm/internlm2-math-base-7b}{Intern-Math} & 7B & - & 31B & 125B & 41.8 & 14.4 & 61.6 & 66.8 & 83.7 & 50.0 & 57.3  & 24.8 & 37.5 & 48.7 \\
% \href{https://huggingface.co/internlm/internlm2-math-base-20b}{Intern-Math} & 20B & - & 31B & 125B & \hlb{65.4} & 30.0 & \hlb{75.7} & 79.3 & \hlb{94.0} & 50.9 & 38.5 & 53.1 & 71.9 & 62.1\\
% \href{https://huggingface.co/deepseek-ai/deepseek-math-7b-base}{DeepSeekMath} & 7B & - & 120B & 500B & {64.1} & \hlb{34.2} & {74.0} & \hlb{83.9} & {92.4} & \hlb{63.4} & \hlb{62.4} & 56.4 & \hlb{84.4} & \hlb{68.4} \\
% \midrule
% \multicolumn{15}{c}{\texttt{Continual Pretraining on Mistral-7B}} \\
% \midrule
% Mistral-CT & 7B & OWM & 14B & 15B & 42.9 & 22.2 & 68.6 & 71.0 & 86.1 & 45.1 & 47.7 & 52.6 & 65.6 & 55.8\\
% -Math & 7B & OWM & 14B & {10.5B} & \hl{66.9} & \hl{31.0} & \hl{77.8} & \hl{79.0} & \hl{93.9} & \hl{49.9} & \hl{58.7} & \hl{54.6} & \hl{84.4} & \hl{66.2}\\
% $\Delta$  & & & & \grey{-30\%} & \blue{+24.0} & \blue{+8.8} & \blue{+9.2} & \blue{+8.0} & \blue{+7.8} & \blue{+4.8} & \blue{+11.0} & \blue{+2.0} & \blue{+18.8} &  \blue{\textbf{+10.4}}\\  
% \bottomrule
% \end{tabular}
% }
% \end{table*}

